DiffLocks: Generating 3D Hair from a Single Image using Diffusion Models

We address the task of generating 3D hair geometry from a single image, which is challenging due to the diversity of hairstyles and the lack of paired image-to-3D hair data. Previous methods are primarily trained on synthetic data and cope with the limited amount of such data by using low-dimensional intermediate representations, such as guide strands and scalp-level embeddings, that require post-processing to decode, upsample, and add realism. These approaches fail to reconstruct detailed hair, struggle with curly hair, or are limited to handling only a few hairstyles. To overcome these limitations, we propose DiffLocks, a novel framework that enables detailed reconstruction of a wide variety of hairstyles directly from a single image. First, we address the lack of 3D hair data by automating the creation of the largest synthetic hair dataset to date, containing 40K hairstyles. Second, we leverage the synthetic hair dataset to learn an image-conditioned diffusion-transfomer model that generates accurate 3D strands from a single frontal image. By using a pretrained image backbone, our method generalizes to in-the-wild images despite being trained only on synthetic data. Our diffusion model predicts a scalp texture map in which any point in the map contains the latent code for an individual hair strand. These codes are directly decoded to 3D strands without post-processing techniques. Representing individual strands, instead of guide strands, enables the transformer to model the detailed spatial structure of complex hairstyles. With this, DiffLocks can recover highly curled hair, like afro hairstyles, from a single image for the first time. Data and code is available at https://radualexandru.github.io/difflocks/

==> fig/fig_results.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{example-image-duck}
    \caption{full page results, test set, in-the-wild, etc}
    \label{fig:result}
\end{figure*}

==> fig/hair_synth_pipeline.tex <==
\begin{figure}
% \captionsetup[subfloat]{labelformat=empty}
\captionsetup[subfigure]{labelformat=empty}
     \centering
     \begin{subfigure}[b]{0.133\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/hair_synth_pipeline/7_initial_e.png}
         \caption{Initial hair}
         % \label{fig:y equals x}
     \end{subfigure}
     % \hfill
     \hspace{-1.2em}% Space between image A and B
     \begin{subfigure}[b]{0.133\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/hair_synth_pipeline/6_just_clumps_e.png}
         \caption{+clumps}
         % \label{fig:three sin x}
     \end{subfigure}
     % \hfill
     \hspace{-1.2em}% Space between image A and B
     \begin{subfigure}[b]{0.133\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/hair_synth_pipeline/3_without_curls_e.png}
         \caption{+curls}
         % \label{fig:three sin x}
     \end{subfigure}
     % \hfill
     \hspace{-1.2em}% Space between image A and B
     \begin{subfigure}[b]{0.133\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/hair_synth_pipeline/0_final_e.png}
         \caption{+fly-away hairs}
         % \label{fig:three sin x}
     \end{subfigure}
    \caption{\textbf{Synthetic pipeline.} The synthetic data pipeline consists of a chain of transformations applied to the hair. The initial hair strands are clumped, curled and noised with different frequencies and strenghts in order to generate realistic hair. Depicted are some of the main transformations applied to the hair. The full pipeline in Blender consists of 58 transformations modeled as Geometry Nodes. Best viewed zoomed in.}
    \label{fig:hair_synth_pipeline}
\end{figure}

==> fig/rebuttal/comparison_hairstep.tex <==
\vspace{-0.05in}
\begin{figure}[h]
	% \small
    % \sffamily

	\centering
	% \tdplotsetmaincoords{-35.3}{0}
	% \tdplotsetrotatedcoords{0}{-45}{0}
	%%%%% CONVOLUTION filter over the vertices
	\begin{tikzpicture}[  ]

     \def\xshift{1.6}
     \def\yshift{0.9}

    %%upper left is at 0,0
    % \node[] (origin) at (0,0) {};

    %base0
    % \node[inner sep=0pt, anchor=south west] (base0) at (-1.2+\xshift*0, 0) {\includegraphics[width=.12\textwidth]{images/rebuttal/density_map/fiennes_2.png}};
    % \node[inner sep=0pt, anchor=south] (def) at (-0.1+\xshift*1, 0) {\includegraphics[width=.12\textwidth]{images/rebuttal/density_map/default.png}};
    %  \node[inner sep=0pt, anchor=south] (def2) at (\xshift*2, 0) {\includegraphics[width=.12\textwidth]{images/rebuttal/density_map/default_density_increase.png}};
    % \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of base0] {RGB Input};
    % \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of def] {Generated hair};
    % \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of def2] {Increased density};



    %density map v2
    \node[inner sep=0pt, anchor=south west] (base0) at (-1.8+\xshift*0, 0) {\includegraphics[width=.12\textwidth]{images/rebuttal/comparison_hairstep/usc_rendered/00150.jpg}};

    %mine
    \node[inner sep=0pt, anchor=south] (h1) at (-0.1+\xshift*1, \yshift) {\includegraphics[trim={6cm 5cm 6cm 3cm},clip,width=.08\textwidth]{images/rebuttal/comparison_hairstep/hairstep/150.jpg}};
    \node[inner sep=0pt, anchor=south] (h2) at (-0.1+\xshift*2, \yshift) {\includegraphics[trim={6cm 5cm 6cm 3cm},clip,width=.08\textwidth]{images/rebuttal/comparison_hairstep/hairstep/150_top.jpg}};
    \node[inner sep=0pt, anchor=south] (h3) at (-0.1+\xshift*3, \yshift) {\includegraphics[trim={6cm 5cm 6cm 2cm},clip,width=.08\textwidth]{images/rebuttal/comparison_hairstep/hairstep/150_back.jpg}};

    \node[inner sep=0pt, anchor=south] (m1) at (-0.1+\xshift*1, -\yshift) {\includegraphics[trim={6cm 5cm 6cm 3cm},clip,width=.08\textwidth]{images/rebuttal/comparison_hairstep/mine/150.jpg}};
    \node[inner sep=0pt, anchor=south] (m2) at (-0.1+\xshift*2, -\yshift) {\includegraphics[trim={6cm 5cm 6cm 3cm},clip,width=.08\textwidth]{images/rebuttal/comparison_hairstep/mine/150_top.jpg}};
    \node[inner sep=0pt, anchor=south] (m3) at (-0.1+\xshift*3, -\yshift) {\includegraphics[trim={6cm 5cm 6cm 2cm},clip,width=.08\textwidth]{images/rebuttal/comparison_hairstep/mine/150_back.jpg}};


    %hairstep
    \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of base0] {USC rendered};
    \node[rotate=90, font=\footnotesize\selectfont, align=center, left = 0.3cm of h1, anchor=north] {Hairstep};
    \node[rotate=90, font=\footnotesize\selectfont, align=center, left = 0.3cm of m1, anchor=north] {Ours};

    
    
    % \node[inner sep=0pt, anchor=south] (def) at (-0.1+\xshift*1, 0) {\includegraphics[width=.12\textwidth]{images/rebuttal/density_map_v2/defaultv4.jpg}};
    % \node[inner sep=0pt, anchor=south] (def2) at (\xshift*2, 0) {\includegraphics[width=.12\textwidth]{images/rebuttal/density_map_v2/increase_density_v4.jpg}};
    % \node[inner sep=0pt, anchor=south] (def3) at (\xshift*3, 0) {\includegraphics[width=.12\textwidth]{images/rebuttal/density_map_v2/increase_density_v4_more_dense3.jpg}};
    % \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of base0] {RGB Input};
    % \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of def] {Generated hair};
    % \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of def2] {Increased density};
    % \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of def3] {Changed map};
    

    %text for the randomizations
     % \node[font=\footnotesize\selectfont, align=left, below = -0.0cm of base0] {Base};
     %%SUUPER HACKY, this actullay makes the text as white so the next node can draw on top
     % \draw [-, ultra thin, ] (2.5, \yshift) -- (6.9, \yshift) node[midway,fill=white, text=white] (unreal_mid) {\small Unreal Engine};

      % \node[font=\footnotesize\selectfont, align=center, below = -0.0cm of u2] (u_text) {\small Unreal Engine\\ real-time(\SI{16}{\milli\second})};

      % %lines
      % \draw [-, ultra thin, ] (2.5, \yshift) -- (u_text.west |- 2.5, \yshift);
      % \draw [-, ultra thin, ] (u_text.east |- 2.5, \yshift) -- (6.9, \yshift);
	\end{tikzpicture}
	\vspace{-0.1in}
	\caption{Hairstep often reconstructs the wrong hair length, especially on the back of the head. }
	\label{fig:comparison_hairstep}
\end{figure}

==> table/quantitative_eval/Hair_01.tex <==
% % base_6_idx_33423
% \begin{figure}
%     \centering

%     % \begin{minipage}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{l rrr | rrr | rrr}
%         \setlength{\tabcolsep}{0pt}
%         & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
%         \textbf{Method} & $2 / 20$ & $3 / 30$ & $4 / 40$ & $2 / 20$ & $3 / 30$ & $4 / 40$ & $2 / 20$ & $3 / 30$ & $4 / 40$ \\
%         \cline{2-10}
%         & \multicolumn{3}{c}{\textbf{Precision}($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall}($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score}($\uparrow$)} \\
%         \hline
%         NeuralHDHair~\cite{wu2022neuralhdhair}	&	27.57	& 47.30	&	57.12	&	22.67	&	44.90	&	63.06	&	24.88	&	46.07	&	59.94	\\
%         HairStep\cite{zheng2023hairstep}	&	32.10	&	52.78	&	65.90	&	20.04	&	35.55	&	47.71	&	24.67	&	42.48	&	55.35	\\
%         Ours	&	49.93	&	\textbf{73.46}	&	\textbf{49.93}	&	\textbf{52.20}	&	\textbf{76.88}	&	\textbf{88.90}	&	\textbf{51.04}	&	\textbf{75.13}	&	\textbf{86.60}	\\
%     \end{tabular}
%     }
%     % \end{minipage}
%     \vspace{0.3cm}

%     % \begin{minipage}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{l rrr | rrr | rrr}
%         \setlength{\tabcolsep}{0pt}
%         & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
%         \textbf{Method} & $2 / 20$ & $3 / 30$ & $4 / 40$ & $2 / 20$ & $3 / 30$ & $4 / 40$ & $2 / 20$ & $3 / 30$ & $4 / 40$ \\
%         \cline{2-10}
%         & \multicolumn{3}{c}{\textbf{Precision}($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall}($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score}($\uparrow$)} \\
%         \hline
%         NeuralHDHair~\cite{wu2022neuralhdhair}	&	27.57	& 47.30	&	57.12	&	22.67	&	44.90	&	63.06	&	24.88	&	46.07	&	59.94	\\
%         HairStep\cite{zheng2023hairstep}	&	32.10	&	52.78	&	65.90	&	20.04	&	35.55	&	47.71	&	24.67	&	42.48	&	55.35	\\
%         Ours	&	49.93	&	\textbf{73.46}	&	\textbf{49.93}	&	\textbf{52.20}	&	\textbf{76.88}	&	\textbf{88.90}	&	\textbf{51.04}	&	\textbf{75.13}	&	\textbf{86.60}	\\
%     \end{tabular}
%     }
%     % \end{minipage}
%     \captionof{table}{}
    
%     \label{tab:quantitative}
%      \vspace{-0.2cm}
% \end{figure}







\begin{figure*}[htbp]
    \centering
    \setlength{\tabcolsep}{8pt} 
    \begin{minipage}{\textwidth}

    
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_6_idx_33423.jpg} 
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
       
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair}	&	27.57	& 47.30	&	57.12	&	22.67	&	44.90	&	63.06	&	24.88	&	46.07	&	59.94	\\
         HairStep\cite{zheng2023hairstep}	&	32.10	&	52.78	&	65.90	&	20.04	&	35.55	&	47.71	&	24.67	&	42.48	&	55.35	\\
         Ours	&	\textbf{49.93}	&	\textbf{73.46}	&	\textbf{84.42}	&	\textbf{52.20}	&	\textbf{76.88}	&	\textbf{88.90}	&	\textbf{51.04}	&	\textbf{75.13}	&	\textbf{86.60}	\\
        \end{tabular}
    \end{minipage}

    \vspace{0mm}

    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_19_idx_41724.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 38.30 & 54.20 & 61.76 & 54.50 & 80.77 & 89.65 & 44.99 & 64.87 & 73.14 \\
            HairStep~\cite{zheng2023hairstep} & 33.40 & 54.09 & 63.08 & 36.42 & 60.63 & 71.23 & 34.84 & 57.17 & 66.91 \\
            Ours & \textbf{89.68} & \textbf{96.70} & \textbf{98.24} & \textbf{86.47} & \textbf{93.82} & \textbf{96.44} & \textbf{88.05} & \textbf{95.24} & \textbf{97.33} \\
        \end{tabular}
    \end{minipage}

    \vspace{0mm}
    
    %base_25_idx_56
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_25_idx_56.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 31.27 & 62.32 & 80.14 & 32.20 & 60.04 & 77.37 & 31.73 & 61.16 & 78.73 \\
            HairStep~\cite{zheng2023hairstep} & 41.17 & 61.83 & 71.11 & 38.43 & 66.04 & 81.06 & 39.76 & 63.87 & 75.76 \\
            Ours & \textbf{63.71} & \textbf{84.26} & \textbf{92.67} & \textbf{62.97} & \textbf{84.77} & \textbf{93.34} & \textbf{63.34} & \textbf{84.51} & \textbf{93.00} \\
        \end{tabular}
    \end{minipage}


    \vspace{0mm}
    %base_66_idx_41697
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_66_idx_41697.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 16.75 & 43.33 & 62.75 & 9.33 & 22.73 & 37.59 & 11.99 & 29.82 & 47.01 \\
            HairStep~\cite{zheng2023hairstep} & 26.50 & 60.19 & 79.40 & 10.14 & 23.01 & 37.34 & 14.67 & 33.29 & 50.80 \\
            Ours & \textbf{29.53} & \textbf{62.11} & \textbf{81.67} & \textbf{34.39} & \textbf{69.56} & \textbf{87.98} & \textbf{31.77} & \textbf{65.62} & \textbf{84.71} \\
        \end{tabular}
    \end{minipage}

    \vspace{0mm}
    %base_67_idx_54
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_67_idx_54.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 16.83 & 31.60 & 43.07 & 20.15 & 42.45 & 62.18 & 18.34 & 36.23 & 50.89 \\
            HairStep~\cite{zheng2023hairstep} & 28.87 & 42.79 & 50.31 & 38.85 & 64.23 & 78.16 & 33.13 & 51.37 & 61.21 \\
            Ours & \textbf{85.73} & \textbf{96.97} & \textbf{99.05} & \textbf{84.34} & \textbf{96.37} & \textbf{98.70} & \textbf{85.03} & \textbf{96.67} & \textbf{98.87  } \\
        \end{tabular}
    \end{minipage}

    \vspace{0mm}
    %base_67_idx_75077
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_67_idx_75077.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 10.60 & 31.98 & 52.94 & 5.45 & 17.77 & 32.98 & 7.19 & 22.84 & 40.64 \\
            HairStep~\cite{zheng2023hairstep} & 6.56 & 21.95 & 40.96 & 3.83 & 10.15 & 19.50 & 4.84 & 13.88 & 26.42 \\
            Ours & \textbf{38.33} & \textbf{71.01} & \textbf{88.46} & \textbf{34.37} & \textbf{65.80} & \textbf{83.83} & \textbf{36.24} & \textbf{68.30} & \textbf{86.08} \\
        \end{tabular}
    \end{minipage}

    \vspace{0mm}
    
    %base_68_idx_83420
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_68_idx_83420.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 9.90 & 24.95 & 40.50 & 10.70 & 24.12 & 38.74 & 10.29 & 24.53 & 39.60 \\
            HairStep~\cite{zheng2023hairstep} & 9.78 & 18.98 & 26.92 & 14.08 & 29.42 & 45.88 & 11.54 & 23.07 & 33.93 \\
            Ours & \textbf{54.17} & \textbf{81.83} & \textbf{92.75} & \textbf{51.87} & \textbf{78.94} & \textbf{90.60} & \textbf{53.00} & \textbf{80.36} & \textbf{91.67} \\
        \end{tabular}
    \end{minipage}

    \vspace{0mm}
    %base_70_idx_75046
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_70_idx_75046.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 17.64 & 31.10 & 41.55 & 21.04 & 43.40 & 59.30 & 19.19 & 36.24 & 48.87 \\
            HairStep~\cite{zheng2023hairstep} & 11.90 & 18.39 & 24.29 & 17.26 & 33.64 & 50.13 & 14.09 & 23.78 & 32.7 \\
            Ours & \textbf{85.82} & \textbf{97.15} & \textbf{85.82} & \textbf{73.10} & \textbf{86.27} & \textbf{90.94} & \textbf{78.95} & \textbf{91.39} & \textbf{94.85} \\
        \end{tabular}
    \end{minipage}

    \vspace{0mm}

    %base_74_idx_91716
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_74_idx_91716.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 11.34 & 21.98 & 34.32 & 8.76 & 19.74 & 27.98 & 9.89 & 20.80 & 30.82 \\
            HairStep~\cite{zheng2023hairstep} & 7.69 & 15.41 & 21.67 & 21.96 & 44.94 & 65.67 & 11.39 & 22.95 & 32.58 \\
            Ours & \textbf{70.03} & \textbf{91.91} & \textbf{97.29} & \textbf{55.16} & \textbf{77.37} & \textbf{87.19} & \textbf{61.71} & \textbf{84.02} & \textbf{91.96} \\
        \end{tabular}
    \end{minipage}

    \vspace{0mm}
    %base_75_idx_58362
    \begin{minipage}{0.12\linewidth}
        \includegraphics[width=\linewidth]{images/evaluation_images/base_75_idx_58362.jpg} 
        % \label{fig:example_image}
    \end{minipage}
    \hfill 
    \begin{minipage}{0.8\textwidth}
        \scriptsize 
        \begin{tabular}{l rrr | rrr | rrr}
            \setlength{\tabcolsep}{0pt}
            \renewcommand{\arraystretch}{3}
            & \multicolumn{9}{c}{\textbf{Thresholds: mm} $/$ \textbf{degrees}} \\
            \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
            \cline{2-10}
            & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
            \hline
            NeuralHDHair~\cite{wu2022neuralhdhair} & 6.38 & 13.38 & 20.47 & 7.85 & 17.39 & 27.23 & 7.04 & 15.12 & 23.37 \\
            HairStep~\cite{zheng2023hairstep} & 4.29 & 9.02 & 13.72 & 7.02 & 17.73 & 31.59 & 5.32 & 11.96 & 19.13 \\
            Ours & \textbf{63.73} & \textbf{86.23} & \textbf{94.16} & \textbf{44.22} & \textbf{67.34} & \textbf{80.17} & \textbf{52.21} & \textbf{75.63} & \textbf{86.60} \\
        \end{tabular}
    \end{minipage}
    \end{minipage}

    \caption{\textbf{Quantitative comparison.}}
    \label{fig:image-quantitative}
\end{figure*}







% \begin{figure*}[htbp]
%     \centering
%     \setlength{\tabcolsep}{1pt}
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         \scriptsize 
%         \begin{tabular}{l rrr | rrr | rrr}
%             
%             & \multicolumn{9}{c}{\textbf{Hair01}} \\
%             \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
%             \cline{2-10}
%             & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
%             \hline
%             NeuralHDHair~\cite{wu2022neuralhdhair} & \textbf{47.91} & 65.07 & 73.76 & 31.59 & 51.10 & 64.63 & 38.00 & 57.12 & 68.73 \\
%             HairStep~\cite{zheng2023hairstep} & 40.88 & 55.99 & 64.07 & 32.16 & 44.96 & 53.15 & 35.50 & 49.06 & 57.20 \\
%             Ours & 43.60 & \textbf{68.30} & \textbf{81.79} & \textbf{34.97} & \textbf{58.27} & \textbf{71.79} & \textbf{38.35} & \textbf{62.41} & \textbf{76.20} \\
%         \end{tabular}

%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.45\linewidth}
%         \centering
%         \scriptsize 
%         \begin{tabular}{l rrr | rrr | rrr}
%             & \multicolumn{9}{c}{\textbf{Hair02}} \\
%             \textbf{Method} & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ & $2/20$ & $3/30$ & $4/40$ \\
%             \cline{2-10}
%             & \multicolumn{3}{c}{\textbf{Precision} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{Recall} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{F-score} ($\uparrow$)} \\
%             \hline
%             NeuralHDHair~\cite{wu2022neuralhdhair} & \textbf{47.91} & 65.07 & 73.76 & 31.59 & 51.10 & 64.63 & 38.00 & 57.12 & 68.73 \\
%             HairStep~\cite{zheng2023hairstep} & 40.88 & 55.99 & 64.07 & 32.16 & 44.96 & 53.15 & 35.50 & 49.06 & 57.20 \\
%             Ours & 43.60 & \textbf{68.30} & \textbf{81.79} & \textbf{34.97} & \textbf{58.27} & \textbf{71.79} & \textbf{38.35} & \textbf{62.41} & \textbf{76.20} \\
%         \end{tabular}
%     \end{minipage}

%     \caption{}
%     \label{fig:}

% \end{figure*}
